Optimized Distribution of Entanglement Graph States in Quantum Networks

Building large-scale quantum computers, essential to demonstrating quantum advantage, is a key challenge. Quantum Networks (QNs) can help address this challenge by enabling the construction of large, robust, and more capable quantum computing platforms by connecting smaller quantum computers. Moreover, unlike classical systems, QNs can enable fully secured long-distance communication. Thus, quantum networks lie at the heart of the success of future quantum information technologies. In quantum networks, multipartite entangled states distributed over the network help implement and support many quantum network applications for communications, sensing, and computing. Our work focuses on developing optimal techniques to generate and distribute multipartite entanglement states efficiently. Prior works on generating general multipartite entanglement states have focused on the objective of minimizing the number of maximally entangled pairs (EPs) while ignoring the heterogeneity of the network nodes and links as well as the stochastic nature of underlying processes. In this work, we develop a hypergraph based linear programming framework that delivers optimal (under certain assumptions) generation schemes for general multipartite entanglement represented by graph states, under the network resources, decoherence, and fidelity constraints, while considering the stochasticity of the underlying processes. We illustrate our technique by developing generation schemes for the special cases of path and tree graph states, and discuss optimized generation schemes for more general classes of graph states. Using extensive simulations over a quantum network simulator (NetSquid), we demonstrate the effectiveness of our developed techniques and show that they outperform prior known schemes by up to orders of magnitude.

==> 20-qc-background.tex <==
\section{QC Background}
\label{sec:background}

\para{Qubit States.}
Quantum computation manipulates \emph{qubits}
analogous to how classical computation manipulates \emph{bits}.  
At any given time, a bit may be in one of two states, traditionally represented by $0$
and $1$.  A quantum state represented by a
\emph{qubit} is a \emph{superposition} of classical
states, and is usually written as $\alpha_0\ket{0} + \alpha_1\ket{1}$,
where $\alpha_0$ and $\alpha_1$ are \emph{amplitudes} represented by
complex numbers and such that $\norm{\alpha_0}^2 + \norm{\alpha_1}^2 = 1$.
%%%%%%%%%%%%%%%%%%%%
Here, $\ket{0}$ and $\ket{1}$ are the standard (orthonormal) 
\emph{basis} states; concretely, they
may represent physical properties such as spin (down/up),
polarization, charge direction, etc.
%%%%%%%%
When a qubit such as above is {\it measured}, it collapses to a 
$\ket{0}$ state with a probability of $\norm{\alpha_0}^2$ and to
a $\ket{1}$ state with a probability of $\norm{\alpha_1}^2$.
%%%%%%%%%%%%%%%%%%%%%
% Representation
%A state of a $2$-qubit  quantum system can be represented as 
%$\alpha_{00}\ket{00} + \alpha_{01}\ket{01} + \alpha_{10}\ket{10} +
%\alpha_{11}\ket{11}$, and 
In general, a state of an $n$ qubit
system can be represented as $\Sigma_{i=0}^{2^n-1} \alpha_i\ket{i}$
 where ``$i$'' in $\ket{i}$ is $i$'s bit representation. 
\eat{($\Sigma_{i=0}^{2^n-1}\norm{\alpha_i}^2=1$)}

\para{Entanglement.}
Entangled states are multi-qubit states that cannot be
"factorized" into independent single-qubit states. E.g., the 
$2$-qubit state $\frac{1}{\sqrt{2}}\ket{00}
+ \frac{1}{\sqrt{2}}\ket{11}$; this particular system is a
\emph{maximally-entangled} state. 
We refer to maximally-entangled pairs of qubits as \epss.
%%%%%%%%%%%%%%%%%%
The surprising aspect of entangled states is that the combined
system continues to stay entangled, even when 
the individual qubits are physically separated by large distances.
This facilitates many applications, e.g., teleportation of qubit
states by local operations and classical information exchange, as
described next.

\para{Teleportation.} Quantum data cannot be \emph{cloned}~\cite{wooterszurek-nocloning,Dieks-nocloning}, i.e., it is not possible to make \emph{independent} copies of arbitrary quantum information.  
Consequently, direct transmission of quantum data is subject to unrecoverable errors, 
as classical procedures such as amplified signals or re-transmission cannot be applied.
%%%%%%%%%%%%%%%%%%%%%%%%%
An alternative mechanism
for quantum communication is \emph{teleportation}, Fig. \ref{fig:teleport_swap} (a), where a qubit $q$ from a node $A$
is recreated in another node $B$ (\emph{while ``destroying'' the original
qubit $q$}) using only classical communication.
However, this process requires that an \eps 
already established over the nodes $A$ and $B$. 
%%%%%%%%%%%%%%%
Teleportation can thus be used to reliably transfer quantum information.
%, as it only involves
%classical transmission and a priori sharing of \eps, 
%each of which can be reliably done.} 
At a high-level, 
the process of teleporting an arbitrary qubit,
say qubit $q$, from node $A$ to node $B$ can
be summarized as follows:
\begin{packedenumerate}
\item an \eps pair $(e_1, e_2)$ is generated over
$A$ and $B$, with  $e_1$ stored at $A$ and
$e_2$ stored at $B$;

\item 
at $A$, a {\it Bell-state measurement} (BSM) operation 
over $e_1$ and $q$ is performed,
and the 2 classical bits measurement output $(c_1 c_2)$ is sent to $B$
through the classical communication channel; 
at this point, the qubits $q$ and $e_1$ at $A$ are destroyed.

\item manipulating the \eps-pair qubit $e_2$ 
at $B$ based on received $(c_1, c_2)$ 
changes its state to $q$'s initial state.
%the qubit $q$ is obtained at $B$
%(i.e., $e_2$ changes into $q$).
\end{packedenumerate}
Depending on the physical realization of qubits and the BSM operation, 
it may not always be possible to successfully generate the 2 classical bits,
as the BSM operation is stochastic.

\begin{figure}
    \centering
    \includegraphics[width=0.40\textwidth]{figures/teleportation_swapping.png}
    \vspace{-0.15in}
  \caption{(a) Teleportation of $\ket{q}$ from $A$ to $B$, while consuming an entangled pair $(e_1, e_2)$. (b) Entanglement swapping over the triplet of nodes $(A, B, C)$, which results in $A$'s qubit entangled with $C$'s qubit. This can be viewed as a teleportation of $e_2$ from node $B$ to $C$.}
  \vspace{-0.25in}
  \label{fig:teleport_swap}
\end{figure}

\para{Entanglement Swapping (\es).} 
Entanglement swapping is an application of teleportation 
to generate \epss over remote nodes. See Fig. \ref{fig:teleport_swap} (b).
If $A$ and $B$ share an \eps  and $B$ teleports its qubit to $C$, then 
 $A$ and $C$ end up sharing an \eps. 
%%%%%%%%
More elaborately, let us assume that $A$ and $B$
share an \eps, and $B$ and $C$ share a separate \eps. 
Now, $B$ performs a  BSM 
on its two qubits and communicates the result to $C$ (teleporting its 
 qubit that is entangled with $A$ to $C$). When $C$ finishes the protocol, it has a qubit
that is an entangled with $A$'s qubit. Thus, an entanglement swapping (\es)
 operation can be looked up as being performed over a triplet of nodes $(A, B, C)$ 
with \eps available 
at the 
two pairs of adjacent nodes $(A, B)$ and $(B,C)$; it results in an \eps over the pair
of nodes $(A, C)$. 

\para{Fidelity: Decoherence and Operations-Driven.}
Fidelity is a measure of how close a realized state is to the ideal. 
Fidelity of qubit decreases with time, due to interaction with the environment,
as well as gate operations (e.g., in \es). 
%%%%%%
Time-driven fidelity degradation is called \emph{decoherence}. 
To bound decoherence, we limit the aggregate time a qubit spends in a quantum memory before being consumed. 
%%%%%%%%
With regards to operation-driven fidelity degradation, 
Briegel et al.~\cite{BreigelEtAl1998} give an expression 
that relates the fidelity of an \eps generated by \es 
to the fidelities of the operands,  in terms of the 
noise introduced by swap operations and the number of link \epss used. The order of the swap operations (i.e., the structure of the 
swapping tree) does not affect the fidelity. 
%%%%%%%%%%%%%%%
Thus, the operation-driven fidelity degradation of the final \eps 
generated by a swapping-tree $T$
can be controlled by limiting the number of leaves of $T$, assuming that
the link \epss have uniform fidelity (as in~\cite{delft-lp}).

Entanglement Purification~\cite[e.g.]{BreigelEtAl1998} and Quantum Error 
Correction~\cite[e.g.]{QEC} have been widely used to combat fidelity 
degradation.  
Our work focuses on optimally scheduling \es operations with constraints
on fidelity degradation, without purification or error correction.

\subsection{Generating Entanglement Pairs (\epss)}
\label{sec:eps}

As described above, teleportation, which is the only viable means of transferring quantum states over long distances, requires an a priori distribution of \epss. 
Thus,   we need efficient mechanisms to  establish \epss across remote QN nodes; 
this is the goal of our 
work.
%\footnote{\blue{One could also do successive {\it teleportation} one-hop at a time, but this is conceptually equivalent to first establishing an a priori \eps between the remote nodes via a left-deep/right-deep swapping tree over local \eps's and then doing the teleportation.}}
%%%%%%%%%%%%%
Below, we start with describing how \epss are generated between adjacent
(i.e., one-hop away) nodes, and 
then discuss how \epss across a pair of remote nodes can be established 
via \ess. 


\para{Generating \eps over Adjacent Nodes.} 
The physical realization of qubits 
determines the technique used for sharing EPs between adjacent nodes. 
The \emph{heralded entanglement} process~\cite{sigcomm20, caleffi} to 
generate an atom-atom \eps between adjacent nodes $A$ and $B$
is as follows:
%entails each node generating an atom-photon entangled pair, 
%followed by
%an \es operation (optical BSM) which entangles the two atoms.} 
\begin{packedenumerate}
    \item 
Generate an entangled pair of atom and a telecom-wavelength photon at node $A$
and $B$.  
%; this is essentially done by exciting atoms (Rubidium (Rb) isotopes) by laser pulses. 
Qubits at each node are generally realized in an atomic form
%that is amenable 
for longer-term storage, while photonic qubits are used for transmission.
%The telecom-wavelength photons are well-suited for transmission over an optical fiber, while the atoms are better suited for memory storage.

\item 
Once an atom-photon entanglement is locally generated
at each node (at the same time), 
the telecom-photons are then transmitted over an optical fiber to a photon-photon/optical BSM device $C$ located in the middle of 
$A$ and $B$ so that the photons arrive at $C$ 
at the same time.

\item 
The device $C$ performs a BSM over the photons, 
and transmits the classical result to $A$ or $B$ to complete \es.
\end{packedenumerate}
%%%%%%
Other entanglement generation processes have been 
proposed~\cite{MuralidharanEtAl2016}; %our evaluation 
%technical development 
%uses the heralded entanglement;
%generation process as in~\cite{sigcomm20, caleffi}; 
%however,
our techniques themselves are independent of how the link \eps are generated.

%To d \eps between adjacent nodes, we can directly generate an \eps at one node and  transmit one qubit of the \eps to the neighbor, with repeated generation and transmission in case of a loss/error.
%%%%%%%%%%%%%%

\para{Generating \eps between Remote Nodes.} 
Now, \eps between non-adjacent nodes connected by a path in the network 
can be established by 
performing a sequence of \ess at 
intermediate nodes; this requires an a priori \eps over 
each of the adjacent pairs of nodes in the path.
%%%%%%%%%%
E.g., consider a path of nodes $x_0, x_1, x_2, x_3, x_4, x_5$, with an \eps 
between every pair of adjacent nodes $(x_i, x_{i+1})$. Thus, each node $x_i$
($1 \leq i \leq 4$) has two qubits, one of which is entangled with $x_{i-1}$ 
and the other with
$x_{i+1}$. Nodes $x_0$ and $x_5$ have only one qubit each.
%%%%%%%%%%%%%%%%%
To establish an \eps 
between $x_0$ and $x_5$, we can perform a sequence of entanglement
swappings (\ess) as shown in Fig.~\ref{fig:tree}. 
\eat{over the following triplet of nodes:
(i) \es over  $(x_1, x_2, x_3)$ to yield an \eps over $(x_1, x_3)$,
(ii) \es over  $(x_1, x_3, x_4)$ to yield an \eps over $(x_1, x_4)$,
(iii) \es over  $(x_1, x_4, x_5)$ to yield an \eps over $(x_1, x_5)$,
(iv) \es over  $(x_0, x_1, x_5)$ to yield an \eps over $(x_0, x_5)$.}
%%%%%%%%%%%%%%%%%%%%%
Similarly, the sequence of \es over the following triplets would also 
work: $(x_2, x_3, x_4)$, $(x_2, x_4, x_5)$, $(x_0, x_1, x_2)$, 
$(x_0, x_2, x_5)$. 
\eat{Note that some of the above \es can happen \ul{in parallel}, e.g.,
$(x_0, x_1, x_2)$ and $(x_2, x_3, x_4)$ 
can happen 
in parallel, as 
they are over separate sets of qubits.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/swapping_tree.png}
    \vspace{-0.1in}
\caption{A swapping tree over a path. The leaves of the tree are the path-links,
which generate link-\epss continuously.}
\vspace{-0.25in}
\label{fig:tree}
\end{figure}

\para{Swapping Trees.}
In general, given a path $P = s \leadsto d$ from $s$ to $d$, 
any complete binary tree (called a {\it swapping tree}) over 
the ordered links in $P$ gives a way to generate an \eps over $(s, d)$.
%%%%%%%%%%%%
Each vertex in the tree corresponds to a pair of network nodes in $P$, 
with each leaf representing a link in $P$. 
%%%%%%%%%%%%%%
Every pair of siblings $(A, B)$ and $(B, C)$ perform an \es over 
$(A,B,C)$  to yield an \eps over $(A,C)$---their parent.
See Fig.~\ref{fig:tree}. 
\emph{Note that subtrees of a swapping tree execute in parallel.}
%%%%%%%%%%%%%%%%%%%%%%%%%%
Different swapping trees over the same path $P$ can have different performance characteristics, as discussed later (see Fig.~\ref{fig:non-balance}).
%In particular, when a swapping tree is used to continuously 
%generate \epss over the root pair, using \epss being generated continuously at
%the links/leaves, different swapping trees can incur very different expected 
%latency in generating \epss, as discussed below. 

\softpara{Expected Generation Latency/Rate of \epss.}
In general, our goal is to continuously generate \epss at some rate using 
a swapping tree, using continuously generated \epss at the leaves. 
The stochastic nature 
of %the physical mechanisms underlying 
\es operations
means that an \eps at the tree's root will be successfully 
generated only after many failed attempts and hence significant latency.
We refer to this latency as the {\it generation latency} of the \eps at the 
root, and in short, just the generation latency of the tree. 
{\eps generation rate} 
is the inverse of its generation latency. Whenever we refer to generation 
latency/rate, we implicitly mean {\it expected} generation latency/rate. 

\para{Two Generation Protocols: \os and \wt}
When a swapping tree is used to (continuously) generate \epss, there are two 
fundamentally different generation protocols~\cite{gisin,tittel-08}. 

\begin{packeditemize}
\item {\it \os Protocol.}  
%In the \os protocol, an \eps (i.e., the corresponding qubits) is \blue{not stored in the memory} to wait for another \eps to be generated, as in the \wt protocol. 
In this model, all the underlying processes, including link \eps generations and atomic
BSMs are synchronized. If all of them succeed then the end-to-end \eps is generated.
%almost instantaneously. 
If {\it any} of the underlying processes fail,
then all the generated \epss are discarded and the
whole process starts again from scratch (from generation of \eps at links).
In the \os protocol, all swapping trees over a given path $P$
incur the same generation latency---thus, here, the
goal is to select an optimal path $P$ (as in~\cite{sigcomm20,delft-lp}).  \eat{Since all underlying processes have to succeed simultaneously to generate an end-to-end EP, these protocols are inherently exponential in the number of nodes in $P$.} 

\item {\it \wt Protocol.} In \wt protocol, a qubit of an \eps 
may wait (in a quantum memory) for its counterpart to become available so that an \es operation can be performed. 
Using such storage, we preclude discarding successfully generated \epss, and 
thus, reduce the overall latency in generation of a root-level \eps. 
E.g., let  $(A,B)$ and $(B,C)$ be two siblings in a swapping tree and \eps for $(A,B)$ is generated first. Then, \eps $(A,B)$ may wait for the \eps $(B,C)$ to be successfully generated. 
Once the \eps $(B,C)$ is generated, the \es operation
is done over the triplet $(A, B, C)$ to generate the \eps $(A,C)$. 
\bleu{If the \eps $(A,C)$ waits beyond a certain threshold, then it may decohere.}   
\end{packeditemize}

\para{Why \wt is Never Worse.} 
The focus of the \os protocol is to avoid qubit decoherence  
due to storage. But it results in very low generation rates
due to a very-low probability of {\it all} the underlying 
processes succeeding at the same time. 
%%%%%%%%%%%%%%%%%%%%%%%%%%
However, since qubit coherence times are 
typically higher than the link-generation latencies,
\footnote{Link generation latencies 
for 5 to 100km links range from about 3 to 350 milliseconds
for typical network parameters~\cite{caleffi}, while coherence times of few
seconds is very realistic (coherence times of several seconds~\cite{Longdell-2005,Fraval-2005} have been shown 
long ago, and more recently, 
even coherence times of several minutes~\cite{dec-13,dec-14} to a few hours~\cite{dec-15,dec-2021} 
have been demonstrated.}
an appropriately designed \wt protocol will always 
yield better generation rates {\it without significantly compromising the fidelity} (see Theorem~\ref{thm:os-wt}). 
The key is to bound the waiting time to limit decoherence
as desired; e.g., in our protocol, we restrict to trees with high expected 
fidelities (\S\ref{sec:problem}), and discard qubits that
"age" beyond a threshold (\S\ref{sec:dec}).
%%%%%%%%%%%
\bleu{Both protocols use the same number of quantum memories (2 per node), though the \wt protocols will benefit from low-decoherence memories; other hardware requirements 
also remain the same.}

\eat{We note that both protocols require the \red{same number of quantum memories}---two 
per node---but \wt protocol benefit from low-decoherence memories; 
other hardware 
requirements are also same.} 
%%%%%%%%%%%%%%%

\begin{theorem}
Consider a quantum network, a path $P$, a swapping-tree $T$ over $P$, a \os protocol $X$, and a \wt protocol $Y$. Protocol $Y$ discards qubits that age (stay in  memory) beyond a certain threshold $\tau$ (presumably, equal to the coherence time). 
%
We claim that $Y$'s \eps generation rate will at least be that of $X$, 
irrespective of $\tau$ and $T$ (as long as it is over $P$), 
while ensuring that \epss generated by $Y$ are formed by non-decohered qubits and the operation-driven fidelity degradation of $Y$ \epss is same as $X$.
\label{thm:os-wt}
\end{theorem}

The above theorem suggests that \wt approach is always a better approach, irrespective of the decoherence time/limitations. See proof in Appendix~\ref{app:os-wt}. 

%In our simulation results, for our settings, \epss generated by our \wt protocol have fidelities comparable to that of the \os protocol; note that the \epss generated by the \os protocol also incur fidelity degradation due to the unavoidable \es operations.
%Note that the \wt approach naturally degenerates to the \os approach when
%the waiting is bounded to zero---as in such as case, all swapping trees over
%a given path would have equal 

%\red{Can the \os model work with no memories? i.e., with "relays"? See Gisin paper.}

\eat{
{\it Paths vs.\ Trees.} When using \os protocol, all swapping trees over a given path $P$
incur the same generation latency. Thus, in the context of \os protocol, the
goal is to select an optimal path $P$ (as in~\cite{sigcomm20,delft-lp}). 
%%%%%
In this paper, we use the \wt protocol, and focus on the selection 
of efficient swapping trees 
with low generation latency
and bounded fidelity. The only other work, to the best
of our knowledge, that uses the \wt protocol, is~\cite{caleffi}.  
However, even that work focuses on selection of paths (in exponential time) and constructs balanced trees over the selected path.
%as it implicitly selects only balanced trees (in exponential time).
%%%%%%%%%%%%
}

==> 4a-one-step-LP.tex <==
\softpara{Hypergraph's vertices $V(H)$ consists of 5 types:}
\begin{enumerate}
  \item Two distinguished vertices \emph{start} and \emph{term}
  \item $avail(x,u,v,y) \ \forall$ $u, v \in V(\texttt{Path})$, $x,y \in V(G) -  V(\texttt{Path})$. Conditions: All non-null values are distinct, and two can be null. To avoid duplicities:  (i) $u < v$ (if both non-null), (ii) if one of $u$ or $v$ is null, then $v$ is null, (iii) if both $u$ and $v$ are null, then $x < y$.

  % Let's discuss $avail(x,u,v,y)$ in terms of some values potentially being $-1$, meaning ``not exist''. \red{Get rid of everything with -1 cases.}
  %   \begin{enumerate}
  %       \item $u = v = -1$. Then $x$ and $y$ must both $\geq 0$. In this case, $avail(x,-1,-1,y)$ means 2-qubit graph state.
  %       \item $u=-1$ and $v\geq 0$. If one of $u$ and $v$ is $-1$, let it always be $v=-1$. Then $x$ and $y$ cannot both $=-1$. 
  %           \begin{itemize}
  %               \item $x\geq 0, y = -1$.  If one of $x$ and $y$ is $-1$, let it be $y=-1$. In this case, $avail(x,u,-1,-1)$ means a single terminal node $u$ extends to a non-terminal node $x$.
  %               \item $x\geq 0, y\geq 0$. 
  %               In this case, $avail(x,u,-1,y)$ means a single terminal node $u$ extends to non-terminal node $x$ on one side, and to $y$ on the other side.
  %           \end{itemize}
  %       \item $u\geq 0, v\geq 0$. Then there is no restriction on $x$ and $y$ being $-1$ or not.
  %       In this case, $avail(x,u,v,y)$ means a path state from ``$u$ to $v$'' with an extension from $u$ to non-terminal $x$ (if $x\geq 0$) and an extension from $v$ to non-terminal $y$ (if $y\geq 0$). 
  %   \end{enumerate}
  \item $\ prod\_fusion\_retain(x,u,v,y), $ and $prod\_fusion\_discard(x,u,v,y) \ \forall$ distinct $u, v \in V(\texttt{Path})$ 
  % meaning a path graph state from ``$u$ to $v$'', with $x,y \in G$ and $\notin V(\texttt{Path})$ meaning an left-side extension to a non-terminal node $x$ and a right-side extension to a non-terminal node $y$. $x$ and $y$ could (both) equal $-1$ meaning there is no extension.
\end{enumerate}

For simplicity, $pfr()$ is short for $prod\_fusion\_retain()$, $pfd()$ is short for $prod\_fusion\_discard()$, and $al()$ is short for $avail()$. 


\softpara{Hypergraph's hyperedges $E(H)$ consists of 6 types:}
\red{Get rid of everything with -1 cases.}

\begin{enumerate}
  \item{[$start$] $e=(\{start\},\{al(u,v)\})\ \forall$ distinct $u,v \in V$}

  \item{[$fusion\_retain$] 
     \begin{enumerate}
         \item $e=(\{al(x,u,i,-1), al(-1,i,v,y)\}, \{pfr(x,u,v,y\})$
         \item $e=(\{al(x,u,-1,-1), al(y,u,-1,-1)\}, \{pfr(x,u,-1,y\})$
     \end{enumerate}
     $\ \forall $ distinct $ u,i,v \in V(\texttt{Path})$}
  
  \item{[$fusion\_discard$] \\
  $e=(\{al(x,u,i,z), al(z,j,v,y)\}, \{pfd(x,u,v,y\})$ \\ $\ \forall $ distinct $ u,i,j,v \in V(\texttt{Path})$ and node $j$ is the terminal node right next to node $i$ in $\texttt{Path}$.
  Above is the case when all values in $avail()$ $\neq -1$ and fusion discard happens at $z$.
  However, recall that some of the values in $avail$ could equal $-1$. So, we consider the following cases:
    \begin{enumerate}
        \item $e=(\{al(x,-1,-1,z), al(z,-1,-1,y)\}, \{pfd(x,-1,-1,y\})$
        \item $e=(\{al(x,u,v,z), al(z,-1,-1,y)\}, \{pfd(x,u,v,y\})$
        \item $e=(\{al(z,-1,-1,x), al(x,u,v,z)\}, \{pfd(z,u,v,y\})$
        \item $e=(\{al(x,u,-1,z), al(z,-1,-1,y)\}, \{pfd(x,u,-1,y\})$
        \item $e=(\{al(x,-1,-1,z), al(z,u,-1,y)\}, \{pfd(x,u,-1,y\})$
    \end{enumerate}
  }
    
  \item{[$pfr\_a$] $e=(\{pfr(x,u,v,y)\},\{al(x,u,v,y)\})$ \\ $\ \forall$ valid $pfr(x,u,v,y)$}
  \item{[$pfd\_a$] $e=(\{pfd(x,u,v,y)\},\{al(x,u,v,y)\})$ \\ $\ \forall$ valid $pfd(x,u,v,y)$}
  \item{[$term$] $e=(\{al(-1,u,v,-1)\},\{term\})$ \\ $u=\texttt{Path}[0],v=\texttt{Path}[-1]$}
\end{enumerate}

==> 4b-two-step-LP.tex <==

\softpara{Hypergraph's vertices $V(H)$ consists of 6 types:}
\begin{enumerate}
  \item 
    $ae(u,v)$ and $ps(u,v) \ \forall$ distinct $u, v \in V$, and $u < v$. \\ 
    $ae(u,v)$ means \underline{a}vailable \underline{E}Ps between node $u$ and $v$ that is ready for future operations. 
    $ps(u,v)$ means EPs between node $u$ and $v$ \underline{p}roduced by \underline{s}wapping.
  \item 
    $ag(\udv)$ and $pf(\udv)\\
    \forall$ distinct $u, v \in V(\texttt{Path}(s\cdotp\cdotp d)))$. \\ $ag(\udv)$ means \underline{a}vailable path \underline{g}raph state \texttt{Path}$(\udv)$ that is ready for future operations. $pf(\udv)$ means path graph state \texttt{Path}$(\udv)$ \underline{p}roduced by \underline{f}usion.
  \item 
    Two distinguished vertices \emph{start} and \emph{term}
\end{enumerate}

\softpara{Hypergraph's hyperedges $E(H)$ consists of 7 types:}
\begin{enumerate}
  \item{[$start$] $e=(\{start\},\{ae(u,v)\}) \\ 
  \forall$ distinct edge $(u,v) \in E$, represent making the link EPs generated between adjacent nodes available.}
  
  \item{[$swap$] $e=(\{ae(u,w),ae(w,v)\},\{ps(u,v)\})$ \\  $\forall$ distinct $ u,v,w \in V$, represent the entanglement swapping operation at node $w$.}
  
  \item{[$ps\_ae$] $e=(\{ps(u,v)\},\{ae(u,v)\})$ \\ $\forall $ distinct $ u,v \in V$, represent making the EPs generated by entanglement swapping available for future operations.}
  
  \item{[$ae\_ag$] $e=(\{ae(u,v)\},\{ag(\udv)\}) $ \\ $\forall $ distinct  $ (u,v) \in E(\texttt{Path}(\udv))$, represent converting the available EPs into available 2-qubit graph states by a local operation (applying H gate on either one of $u$ or $v$). If $u > v$ in $ag(\udv)$, then $ae(u,v)$ becomes $ae(v,u)$.}
  
  \item{[$fusion$] $e=(\{ag(u\cdotp\cdotp w), ag(w\cdotp\cdotp v)\},\{pf(\udv)\})$ \\ $\ \forall $ distinct $ u,w,v \in V(\texttt{Path}(\udv))$, represent fusion\CZ{talk about the fusion retain operation somewhere} operation at node $w$.}
  
  \item{[$pf\_ag$] $e=(\{pf(\udv)\},\{ag(\udv)\})$ \\ $\ \forall$ distinct $ u,v \in V(\texttt{Path})$, represent making the path graph state generated by fusion operation available for future operations.}
  
  \item{[$term$] $e=(\{ag(s\cdotp\cdotp d)\},\{term\})$}
\end{enumerate}


==> 5a-tree-LP.tex <==
\softpara{Hypergraphs's vertices $V(H)$ consists of 7 types:}
\begin{enumerate}
  \item Two distinguished vertices \emph{start} and \emph{term}
  \item $avail(u,v)$ and $prod\_swap(u,v)\ \forall $ distinct $ u,v \in V$ 
  \item $avail3(p,u,v,x) \ \forall p \in V(\texttt{Tree})$ with children ``$u$ to $v$'', where $u \leq v$. The ascending order assumption for children remains the same.
  $x$ means an extension to node $x$ and $x\notin subtree(p)$. 
  If there is no extension, then $x=-1$.
  \item $prod\_fusion1(p,u,v,x) \ \forall p \in V(\texttt{Tree}) $ with children ``$u$ to $v$'', where $u < v$.
  \item $prod\_fusion3(p,u,v,x) \ \forall p \in V(\texttt{Tree})$ that has both children and a parent, and the children are ``$u$ to $v$'' where $u \leq v$.
\end{enumerate}

For simplicity, $ps()$ is short for $prod\_swap()$, $pf1()$ is short for $prod\_fusion1()$, and $pf3()$ is short for $prod\_fusion3()$  

\softpara{Hypergraph's hyperedges $E(H)$ consists of 10 types:}
\begin{enumerate}
  \item{[$start$] $e=(\{start\}, \ \{avail(u,v)\})  \ \forall $ distinct $ u,v \in V$}
  \item{[$swap$] $e=(\{avail(u,w),avail(w,v)\},\ \{ps(u,v)\})$ \\  $\forall$ distinct $ u,v,w \in V$}
  \item{[$ps\_a$] $e=(\{ps(u,v)\},\ \{avail(u,v)\})$ \\ $\forall $ distinct $ u,v \in V$}
  \item{[$a\_a3$] $e=(\{avail(u,v)\},\ \{avail3(u,v,v,-1)\}) $ \\ $\forall $ distinct  $ (u,v) \in E(\texttt{Tree}), parent(v) = u$ and $v$ is a leaf node in $\texttt{Tree}$}
  \item{[$fusion1$] $e=(\{avail3(p,u,i,x), \ avail3(p,j,v,-1)\},$ $ \{pf1(p,u,v,x)\})$  $\ \forall p \in V(\texttt{Tree})$ that has two or more children, $u \leq i < j \leq v$, and $j$ is right after $i$ in the children's ascending order.
  $x$ is allowed to be -1, meaning no extension.}
  \item{[$fusion3$] $e=(\{avail3(p,u,v,x), \ avail(x,y)\}, $ $ \{pf3(p,u,v,y)\})$  $\ \forall p \in V(\texttt{Tree})$ that has both children and a parent. The children are from ``$u$ to $v$'', where $u \leq v$.
  If $x=-1$, then $avail3(p,u,v,-1)$ fuses with $avail(p,y)$ and generates $avail3(p,u,v,y)$}
  \item{[$pf1\_a3$] $e=(\{pf1(p,u,v,x)\},\{avail3(p,u,v,x)\})$ \\ $\ \forall$ valid $pf1(p,u,v)$}
  \item{[$pf3\_a3$] $e=(\{pf3(p,u,v,x)\},\{avail3(p,u,v,x)\})$ \\ $\ \forall$ valid $pf3(p,u,v,x)$}
  \item{[$a3\_a3$] $e=( \{ avail3(p,a,z,p2) \}, \{ avail3(p2,p,p,-1)  \} )$  $\forall p \in V(\texttt{Tree})$ that has both children and a parent, and $parent(p) = p2$, and ``$a$ to $z$'' means that subtree $p$ is complete.}
  \item{[$term$] $e=(\{avail3(p,a,z,-1))\},\{term\})$, where $p$ is the root of $\texttt{Tree}$, and $avail3(p,a,z,-1)$ is complete without extension.}
\end{enumerate}

==> 5c-eaten.tex <==

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/tree-state.png}
%     \caption{\red{A tree graph state spanning nodes $[0,1,3,4,5,7]$ denoted as $\texttt{Tree}(0,1\cdotp\cdotp 4)$.}}
%     \label{fig:tree-state}
% \end{figure}

% \begin{definition}{Tree Graph State}
% \label{defn:tree-state}
% A {\it tree graph state} is a graph state with a tree graph, and a mapping of qubits to network nodes.
% \end{definition}

% \begin{observation}
% \blue{Starting off with link-layer EPs, and using XXXX fusion operations (with the obvious restrictions XXX), the number of intermediate states that can be obtained is exponential in the number of network nodes.}
% \end{observation}



\subsection{\textbf{Hypergraph for a Tree Graph State}}

Given a QN and a single tree graph state $\texttt{Tree}$, we construct a hypergraph 
that represents the set of all possible ways to generate the $\texttt{Tree}$.
Given a QN represented as an undirected graph $G=(V,E)$ and a $\texttt{Tree}$, its \emph{ST-hypergraph} is a hypergraph $H$ constructed as follows (see Fig. \ref{fig:lp-2step-path}). 
$\texttt{Tree}$ is represented by a \magenta{tree data structure} and $V(\texttt{Tree}) \subseteq V, E(\texttt{Tree}) \subseteq E$. 
% All pairs of vertices below are \magenta{unordered pairs}.

\para{Hypergraph Vertices.}
\begin{enumerate}
  \item Two distinguished vertices \emph{start} and \emph{term}
  \item $avail(u,v)$ and $prod\_swap(u,v)\ \forall $ distinct $ u,v \in V$ 
  \item $avail2(u,v)$ \\ $ \ \forall $ distinct  $ (u,v) \in E(\texttt{Tree}) $ and $parent(v) = u$
  \item $avail3(p,u,v) \ \forall p \in V(\texttt{Tree})$ with children ``$u$ to $v$''. Let the children of $p$ be sorted in ascending order by the vertex index. 
  $u$ and $v$ are the children vertex indexes where $u \leq v$.
  If a parent $p$ has $n$ number of children, then the number of $avail3(p,u,v)$ for $p$ is $\frac{(n+1)n}{2}$.
  \item $prod\_fusion1(p,u,v) \ \forall p \in V(\texttt{Tree}) $ with children ``$u$ to $v$''. Here, the difference compared with $avail3(p,u,v)$ is that $u$ is strictly smaller than $v$, i.e., $u < v$.
  \item $prod\_fusion2(p,u,u) \ \forall u \in V(\texttt{Tree})$ that has both children and a parent, and $parent(u) = p$.
\end{enumerate}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/LP-2step-tree.png}
%     \caption{The hypergraph for generating the tree graph state in Fig.~\ref{fig:tree-state}. \red{Remove -- replace it by a "conceptual" idea.}}
%     \label{fig:lp-2step-tree}
% \end{figure}

\para{Hypergraph's Hyperedges.} TWO STEPS.
\begin{enumerate}
  \item{[$start$] $e=(\{start\}, \ \{avail(u,v)\})  \ \forall $ distinct $ u,v \in V$}
  \item{[$swap$] $e=(\{avail(u,w),avail(w,v)\},\ \{ps(u,v)\})$ \\  $\forall$ distinct $ u,v,w \in V$}
  \item{[$ps\_a$] $e=(\{ps(u,v)\},\ \{avail(u,v)\})$ \\ $\forall $ distinct $ u,v \in V$}
  \item{[$a\_a2$] $e=(\{avail(u,v)\},\ \{avail2(u,v)\}) $ \\ $\forall $ distinct  $ (u,v) \in E(\texttt{Tree}), parent(v) = u$}
  \item{[$a2\_a3$] $e=(\{avail2(u,v)\},\ \{avail3(u,v,v)\}) $ \\ $\forall $ distinct  $ (u,v) \in E(\texttt{Tree}), parent(v) = u$ and $v$ is a leaf node in $\texttt{Tree}$}
  \item{[$fusion1$] $e=(\{avail3(p,u,i), \ avail3(p,j,v)\},$ $ \{pf1(p,u,v)\})$  $\ \forall p \in V(\texttt{Tree})$ that has two or more children, $u \leq i < j \leq v$, and $j$ is right after $i$ in the children's ascending order.}
  \item{[$fusion2$] $e=(\{avail3(u,a,z), \ avail2(p,u)\}, $ $ \{pf2(p,u,u)\})$  $\ \forall u \in V(\texttt{Tree})$ that has both children and a parent. Here, $avail3(u,a,z)$ is complete and rooted at $u$. Being complete means $a$ is $u$'s child with smallest index, and $z$ is $u$'s child with largest index, $a \leq z$.}
  \item{[$pf1\_a3$] $e=(\{pf1(p,u,v)\},\{avail3(p,u,v)\})$ \\ $\ \forall$ valid $pf1(p,u,v)$}
  \item{[$pf2\_a3$] $e=(\{pf2(p,u,u)\},\{avail3(p,u,u)\})$ \\ $\ \forall$ valid $pf2(p,u,u)$}
  \item{[$term$] $e=(\{avail3(p,a,z))\},\{term\})$, where $p$ is the root of $\texttt{Tree}$, and $avail3(p,a,z)$ is complete.}
\end{enumerate}

\blue{discuss the meaning of hypergraph...}
\vspace{1in}



\para{LP formulation.} 
\blue{Same as before, except -- fusion probabilities.}
% \begin{itemize}

%     \item \textbf{Variables:} $z_e$, for each hyperedge $e$ in $H$, represents the entanglement generation rate over the (one or two) node-pair in $e$'s tail. \CZ{removed duplication}

%     \item \textbf{Capacity Constraints:} $z_e \in R^+$ for all hyperedges $e$ in $H$. Each node $i$ in the quantum network has an atom-photon pair generation capacity constraint.
%      $$  1/t_g \geq \sum_{x \in E(i)}  z_{e(x)} / (p_g^2 p_e^2 p_{ob}) \quad \forall i \in V  $$
%     Above $e(x)$ is the hyperedge in $H$ of the form $(start, avail(x))$ where $x \in E(i)$ is an edge in $G$ that comprises node $i$.

%     \item \textbf{Flow Constraints,} which vary with vertex types. Below, we use notations $out(v)$ and $in(v)$ to represent outgoing and incoming hyperarcs from $v$. 

%     \begin{itemize}
%         \item For each vertex $v$ s.t. $v=avail(\cdot)$ or $v=avail2(\cdot)$ or $v=avail3(\cdot)$:
%               $$ \sum_{e \in in(v)}  z_e = \sum_{e' \in out(v)} z_{e'} $$
%         \item For each vertex $v$ s.t. $v=prod\_swap(\cdot)$:
%               $$ \sum_{e \in in(v)} (\frac{2}{3} p_b)z_e = \sum_{e' \in out(v)} z_{e'} $$
%         \item For each vertex $v$ s.t. $v=prod\_fusion1(\cdot)$:
%               $$ \sum_{e \in in(v)}  (\frac{2}{3}p_{f1}) z_e  = \sum_{e' \in out(v)} z_{e'} $$
%         \item For each vertex $v$ s.t. 
%         $v=prod\_fusion2(\cdot)$:
%               $$ \sum_{e \in in(v)}  (\frac{2}{3}p_{f2}) z_e  = \sum_{e' \in out(v)} z_{e'} $$
%     \end{itemize}

%     \item \textbf{Objective}: Maximize $\sum_{e \in in(term)} z_e$
    
% \end{itemize}


The above LP formulation is succinct\CZ{better word? Words like simple and easier to understand}. 
The succinctness comes from two assumptions:
\begin{enumerate}
    \item Get all the needed remote EPs ready first (possibly via swapping), and then creating the tree graph state via fusion. 
    There is a ``barrier'' between the swapping step and the fusion step.
    The fourth type of hyperedge in the previous subsection, i.e., $a\_a2$, implements this barrier.
    \item $fusion1$ and $fusion2$ collaborate in a way that $fusion1$ generates a complete subtree state first, and then $fusion2$ grows the height of the complete subtree state by one. 
    So there is also a ``barrier'' between the two fusion operations and the barrier can looked upon as the generation of a complete subtree state.
\end{enumerate}


=




Note that the above hypergraph actually has included the functionality of $avail2$ and $fusion2$ that we attempted to remove.
So adding back $avail2$ and $fusion2$ won't affect the correctness and won't improve the performance, while only adding redundancy.

\blue{Conditional performance guarantee.
One important assumption we made is that while generating the $avail3(p,u,v)$, we assumed $p$'s children are sorted in ascending order by the child's vertex index from $u$ to $v$.
This assumption allows us to express the combination of children using two indexes $u$ and $v$, and decrease the number of $avail3$ from exponential to $O(n^2)$.
}
Under the assumption, our improved LP is \red{near-optimal?} \CZ{It didn't completely get rid of the remote EP}


% For clarity,  we ignore the node and fidelity constraints for now, and
% incorporate them later in \S\ref{sec:fidelity}.

% \para{Basic Idea.}
% The \gffull (\gf) algorithm, like the 
% previous \fro algorithm, 
% also builds bigger and bigger \ghz states from smaller \ghz states until the desired \ghz state is created---but, unlike the \fro algorithm, it may also involve the 
% non-terminal nodes beyond the \epss generation and hence 
% may use \fd operations too. 
% %%%%%%
% Thus, \gf is fundamentally a more general (i.e., less restrictive) algorithm than 
% the \fro algorithm, and hence, has the potential to outperform the \fro algorithm 
% if designed effectively. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%
% At a high level, the \gf algorithm first selects a set $\edgeSet$ of 
% network links (node pairs)
% over which to generate
% the link \epss, and then, constructs an efficient fusion tree over $\edgeSet$.
% %%%
% Since the 
% \epss over $\edgeSet$ must yield (via fusion operations) a \ghz state over the given 
% terminals, the set of links $\edgeSet$
%  must form a connected graph and include the terminals. Thus, the \gf algorithm consists of the following two high-level steps (see Fig~\ref{fig:gf}).
% \begin{enumerate}
%     \item Select the ``best'' Steiner tree $\SteinerTree$ in the original network graph 
%     over the given set of terminals 
%     $\Terminals$. Here, the Steiner tree is essentially a subgraph (not necessarily induced) that is connected and includes the terminals. 
%     \item Construct an efficient fusion tree over the links/edges in $\SteinerTree$. The fusion tree essentially generates \ghz states from the \epss over the links in $\SteinerTree$.
% \end{enumerate}
% Below, we develop a near-optimal algorithm for the first step and an efficient heuristic for the second, as described below.

% \para{1. Selecting the ``Best'' Steiner Tree.}
% Here, we develop an optimal algorithm to find the best Steiner tree $\SteinerTree$ 
% in the given network graph, based on an appropriately define objective function. 
% In graph theory, a Steiner tree in 
% a given graph $G=(V, E)$ for a set of terminals $V' \subseteq V$ is a subgraph (not necessarily induced) 
% in $G$ that is a tree and contains 
% all the terminals in $V'$. 
% %%%%%%%%%%%%%%%%%
% In our context, we want to construct a Steiner tree $\SteinerTree$ in the network graph 
% that includes the set of terminals $\Terminals$. Ideally, the optimization objective should be
% to construct a Steiner tree that yields a fusion tree of minimum \ghz generation latency 
% over its links. Such an optimization objective is however intractable to optimize, since
% it is even intractable to compute an optimal fusion tree over a {\it given} Steiner tree.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Thus, we first derive a simpler optimization objective for a Steiner tree, which is simple  
% as well as reflective of the \ghz generation latency 
% of an efficient fusion tree over the Steiner tree. 

% \softpara{Optimization Objective.}
% To define an optimization objective for a given Steiner tree $\SteinerTree$,
% we need to first estimate the \ghz generation latency 
% of an efficient fusion tree, that we can design an algorithm to construct, 
% over the links in $\SteinerTree$. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% As motivated and described in the second step later, we use a 
% a {\it balanced} binary\footnote{Note that our fusion operations are binary, and hence, the fusion trees in our context are binary trees.} tree over the links in $\SteinerTree$ 
% as the fusion tree to generate the desired \ghz state. 
% %%%%%%%%%%%%%%%%%%%%%%
% Thus, we define the optimization objective for a Steiner tree 
% $\SteinerTree$ by estimating the \ghz generation
% latency of an appropriate balanced fusion tree over $\SteinerTree$.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Consider a given Steiner tree $\SteinerTree$ and a 
% ``balanced'' fusion tree $\fusionTree$ over it.
% We define the objective function $B(\SteinerTree)$ as 
% the \ghz generation latency due to 
% $\fusionTree$ which can be derived as follows.
% \begin{equation}
% B(\SteinerTree) = p^{d}N + [(p^d-1)/(p-1)](\ft + \ct)/\fp \label{eqn:balanced-ft} 
% \end{equation}
% where $p = 3/(2\fp)$ and $d$ and $N$ are defined as follows.
% Let $x$ be the link with highest generation-latency in $\SteinerTree$; then, $N$ is $x$'s  generation latency and $d$ is its depth in the balanced fusion tree $\fusionTree$.
% %%%%%%%%%%%%%%%%%%%%%
% For a balanced fusion tree, it is easy to see that $d$ is either 
% $\lceil(\log_2 |\SteinerTree|)\rceil$ or 
% $\lfloor(\log_2 |\SteinerTree|)\rfloor$, but for simplicity 
% we assume $d$ to be just $\lceil(\log_2 |\SteinerTree|)\rceil$
% to avoid defining $B(\SteinerTree)$ in terms of the exact structure of \SteinerTree.


% Derived from the closed-form formula of calculating a swapping tree latency in our prior work~\cite{swapping_trees22}, 
% So, the generation latency $L(\Steinerseet)$ for a tree $\Steinerseet$ is given by 
% $L(d)$, the generation latency of the fusion tree's root at a distance
% of $d$ from the bottleneck link $L^*$, and is equal to: 
% $$L(\Steinerseet) = L(d) =\pp^{d}T_{L^*} + [(\pp-1)/(\pp^{d}-1)](\ft + \ct)/\fp$$ where 
% $\pp = 3/(2\fp)$ and $d = \lceil(\log_2 |\Steinerseet|)\rceil$.
% Note that, the final fusion tree structure and its latency may be different than this value. We are interested in this value as it is a good constant-cost approximation to the exponential calculation of the fusion trees.

% \softpara{Selecting a Near-Optimal Steiner Tree.}
% Note that the above objective function for a Steiner tree $\SteinerTree$
% depends on only two parameters of $\SteinerTree$: (i) Number of links in $\SteinerTree$, 
% and (ii) The maximum \eps generation latency of a link in $\SteinerTree$. 
% %%%%%%%%%%%%%%
% In addition, it is easy to see that, for a {\it given/fixed} maximum edge-latency, a Steiner tree's objective value decreases with the decrease in the number of links in it.
% %%%%%%%%%%%%%%%%%%
% Thus, for each potential value of maximum edge-latency $l$, we construct a subgraph $G_l$, of original network graph, consisting of links with \eps generation latencies lower than $l$, 
% and then construct a minimum-size Steiner tree $S_l$ in $G_l$. 
% %%%%
% Since there are only a polynomial number of links and thus only a polynomial number of 
% potential $l$ values, we can do the above for each potential $l$ value and pick the best 
% Steiner tree $S_l$. 
% %%%%%%%%%%%
% To compute the minimum-size Steiner tree in a given $G_l$, 
% we can use a well-known 2-approximate algorithm~\cite{kou1981fast}. 
% %%%% 
% The above overall algorithm thus constructs a Steiner tree whose objective value is
% at most 2 times the optimal objective value.

% \para{2. Balanced Fusion Tree Over the Steiner-Tree Links.}
% Having constructed a Steiner tree $\SteinerTree$ over the given terminals, 
% we now need to create
% an efficient fusion tree over the links in $\SteinerTree$---to create the desired \ghz states 
% from the generated \epss over the links, using fusion operations. 
% %%%%%%%%%%%%%%%%%%%%%%%%%
% The exponential-time DP algorithm used to construct a fusion tree in the \fro algorithm 
% is not feasible here, since the number of links in our Steiner tree can be much larger 
% than the number of terminals--and in general, can be as large as the quantum network size. 
% %%%%%%
% Thus, here we design an efficient polynomial-time heuristic based on a divide-and-conquer
% strategy. 
% %\blue{Constructing an optimal fusion tree is NP-hard?} 
% Our proposed 
% heuristic consists of the following three high-level steps. 

% %%%%%%%%%%%%%%%%%%%
% \begin{enumerate}
%     \item Divide the given Steiner tree \SteinerTree with terminals $\Terminals$ into two near-disjoint (with only one node $c$ in common) and approximately ``equal'' subtrees $\SteinerTree_r$ and $\SteinerTree_l$.  We consider two measures of equality---equal in size or in estimated generation latency---and discuss these measures and schemes in detail below. 
%     \item Recursively compute a fusion tree $\fusionTree_r$ ($\fusionTree_l$) for the
%     subtree $\SteinerTree_r$ ($\SteinerTree_l$). The fusion tree $\fusionTree_r$ ($\fusionTree_l$) should be such that the generated \ghz state is over the set of terminals from \SteinerTree in $\SteinerTree_r$ ($\SteinerTree_l$) and the common
%     node $c$.\footnote{Note that subtree is associated with a set of subtree-terminals of its own, which may include nodes not in the original set of terminal $T$.}
%     \item Create a fusion tree with a root $R$ and its two children as $\fusionTree_r$ and $\fusionTree_l$. The root $R$ represents a fusion operation at the node $c$ common to the subtrees $\SteinerTree_r$ and $\SteinerTree_l$. If $c \in \Terminals$, then a \fr operation is used at $c$, else a \fd operation is used. 
% \end{enumerate}

% \input{figures/gf_partition.tex}
% \softpara{Division into Equi-Size Subtrees.}
% Dividing a tree into two equal-sized subtrees may not be straightforward---e.g., consider a star tree. Note that in our context we need to have one node in common between the subtrees, to facilitate a fusion operation over the \ghz states generated from the subtrees. 
% %%%%%%%%%%%%%%%%%%%
% Our heuristic considers each possible common node $c$, 
% and considers dividing the tree into almost-equi-sized
% subtrees with $c$ as the common node. Consider a node $c$ in the given tree, and let $c$'s degree be $m$.  Let $s_1, s_2, \ldots, s_m$ be the sizes of the subtrees of $c$ when we visualize the given tree as rooted at $c$.
% %%%%%%%%%%%%%%%%%%%
% To create almost-equal division of the given 
% tree into two subtrees with $c$ as the common node, we need to just
% partition the set $\{s_i\}$ into two subsets of almost equal sum; this is
% the well-known NP-hard {\tt Partition} problem which has a well-known 
% pseudo-polynomial optimal algorithm based on dynamic programming. 
% %%%%%%%
% We repeat the above for each node $c$ in the tree, 
% and pick the best division into sub-trees; here, the best division is the
% one with minimum difference in the sub-tree sizes. 
% See Fig~\ref{fig:gf_division}(a).

% {\it Equal-Latency Division.}
% To divide a tree into two subtrees that would yield fusion trees of almost-equal generation latencies, we use a similar approach as above---except for the calculation of the $s_i$ values. For equi-latency division, $s_i$ should be an estimate of the generation latency 
% of the envisioned/optimal fusion tree over the $i^{th}$ subtree. 
% %%%%%%%%%%%%%%
% Thus, to determine $s_i$, we assume the fusion tree to be a balanced binary tree, and then, use Eqn.~\ref{eqn:balanced-ft} to estimate the \ghz generation latency. See Fig~\ref{fig:gf_division}(b).





% \red{Enumerate the three steps.} \blue{Essentially, at the highest-level, we divide the given (Steiner) tree into two almost-disjoint (i.e., share one node) subtrees such that they are approximately/almost ''equal'', recursively compute the best fusion trees for each of the subtrees, and finally, fuse them using a fusion-retain or fusion-discard operation depending upon whether the common node is a terminal or not.} 
%%%%%%%%%%%%%%%%%
% Below, we give two different divide-and-conquer schemes based on the above idea, with two different definitions of equality of subtrees. 



% In the first step, we want to select a set of link-level edges $\Steinerseet$ whose generated \epss can be used through a sequence of fusion-retain and fusion-discard operations to form the desired \ghz state .
% Note that the set of the link-level edges $\Steinerseet$, just like the terminal-pairs set in FRO algorithm, should be such that they are "connected" and cover all the terminals. The difference, however, is that we compute, in FRO algorithm, a minimum spanning tree in a complete graph while we want to manipulate the original network graph $G=(V, E)$ to select link-level edges $\Steinerseet$.
% This is a general version of minimum spanning tree where a set of edges $\Steinerseet\in E$ is selected such that a subset of nodes $T\in V$, instead of ALL the nodes, is connected. In graph theory, such set of edges is called Steiner tree and it is solved based on an optimization metric. e.g. Sum of weights of the selected edges $\Steinerseet$.
% The Steiner tree selection problem is itself an NP-hard problem and non-linear fusion tree latency calculations make it even harder.
% To compute a tree that connects ALL the terminals, we used Minimum Spanning Tree algorithm in the previous section.
% Minimum Spanning Tree is an optimal, in terms of overall latency of the connecting edges, way to connect ALL nodes in a graph.
% We achieved this by converting the graph, with the aid of ALL pairs shortest swapping trees, into a one that have only terminals as vertices.
% We can no longer use this approach as we do not want to use bipartite routing.
% The problem of finding the best tree, based on a metric like overall latency, that connects all the terminal, and possibly some other nodes, is a variant of the famous \textit{Steiner Tree}. \blue{It is a variant as the minimum overall latency tree may not lead to the best fusion tree.}















% \softpara{Edge-Balanced Fusion Tree.} 
% In this section, we propose a technique that can be used for both Edge-Balanced and Latency-Balanced approaches.
% We describe the technique for Edge-Balanced fusion tree computation and point out the modifications required for Latency-Balanced fusion tree computation.

% Given a Steiner tree $\Steinerseet$, the goal is to find a node that can divide the whole tree into two almost equal sub-\ghz states. This node will be responsible to perform the last fusion operation.
% The fusion operation can be either retain or discard depending on whether the fusing node itself is part of the final \ghz state. Note that the selected node has to definitely be part of both sub-\ghz states regardless of its final position; this is because this node has to own two qubits, one for each sub-state, to be able to perform the fusion operations.

% To find this node, we do an exhaustive search among all the nodes $V_{\Steinerseet}$ in the tree $\Steinerseet$. For each node $v\in V_{\Steinerseet}$, we first calculate the path and its length each of the node's branches has $\PP_{v}=\{P_1, P_2, ..., P_m\}$, assuming node $v$ is the root for the fusion tree. Here, $m$ is the degree of node $v$ in the tree $\Steinerseet$.
% This can be done by a simple graph traversal algorithm.  
% Now and given the path length of each branch $P_v$, we cluster all the branches into two clusters $S_l$ and $S_r$ such that $S_l \cup S_r = \PP_v$, $S_l \cap S_r=\emptyset$, and the difference between the total number of edges, in each cluster, is minimized $|S_l| - |S_r|$.
% We use a DP approach to find the best set of cluster-pair. \red{Should we explain this DP? We can say we try all possible combinations for simplicity}
% Among all the nodes in the tree, we select the one that has the minimum such value.
% We recursively repeat this process for each sub-\ghz state till we reach to the link-layer edges.

% \softpara{Latency-Balanced Fusion Tree.} 
% To modify the above approach for the Latency-Based, we include the latency bottleneck, the one with the maximum latency, of each branch as well $L_v^*=\{l_1^*, l_2^*, ..., l_m^*\}$. 
% Given $\PP_{v}$ and $L_v^*$, we can simply use the above closed-form formula to calculate the latency of each cluster. Note that the total number of edges of each cluster and the largest bottleneck are used for fusion latency calculations.




% In this section, we develop another algorithm that is exclusively designed to generate and distribute \ghz states without relying on bipartite routing. Due to the problems mentioned, the FRO approach described in the section~\S\ref{sec:fusion_retain} might not be a good approach in some cases.
% The very obvious problem is that bipartite algorithms are designed implicitly assuming there is no other active \epss generation happening. 
% So, the combined case of multiple bipartite routes might not perform the best due to possible ignored intersections.
% Another restriction with the FRO approach is that the fusion operations are performed only in the terminals of a \ghz state.
% \ghz states, however, have an interesting property where one of the entangled node can do some special measurements and detach itself from the entangled state; the remaining entangled nodes would still form a \ghz state, with the number of nodes one less than the original one. 
% These two observations motivate us to come up with a general approach where non-terminal nodes are also allowed to participate in the formation of the required \ghz state. 
% In another word and by allowing other nodes to perform fusion operations, we do not have to create \epss between a pair of terminals first; there might be some nodes, possibly somewhere between the two states, that better breaks down a \ghz state into smaller ones. 
% This node will share two qubits one for each sub-\ghz state, fusing them, and with the aid of $X$ basis measurement detach itself to form the required \ghz state. \red{a figure showing a case that this approach might be better??}
% Overall, the algorithm in this section differs in two things with the FRO: (i) computing the tree that connects the terminals, and (ii) computing the fusion tree over the connecting tree.
% We describe both steps in the following.





% Although the Steiner tree selection problem is NP-hard, there are some approximation solutions that provide good results in practice. 
% Naively, selecting the Steiner tree in the original graph and computing a fusion tree over it may not lead to a good solution as  the latency of a fusion tree depends on both links latency and the number of links (or equivalently the height of the tree). To partially address this problem, we compute different Steiner trees and picks the one that gives the minimum latency. 
% The idea is to try both tall trees with low links latency and shallow trees with high links latency.
% We perform an exhaustive search over all possible Steiner tree solutions.


% To make this approach work, we need to have a way to compare the generation latency of different Steiner trees.
% As discussed before, there are exponential ways of constructing fusion trees over a given tree.
% Derived from the closed-form formula of calculating a swapping tree latency in our prior work~\cite{swapping_trees22}, we, at this step, assume the final fusion tree, of a Steiner tree, is an edge-balanced fusion tree.
% So, the generation latency $L(\Steinerseet)$ for a tree $\Steinerseet$ is given by 
% $L(d)$, the generation latency of the fusion tree's root at a distance
% of $d$ from the bottleneck link $L^*$, and is equal to: 
% $$L(\Steinerseet) = L(d) =\pp^{d}T_{L^*} + [(\pp-1)/(\pp^{d}-1)](\ft + \ct)/\fp$$ where 
% $\pp = 3/(2\fp)$ and $d = \lceil(\log_2 |\Steinerseet|)\rceil$.

% Note that, the final fusion tree structure and its latency may be different than this value. We are interested in this value as it is a good constant-cost approximation to the exponential calculation of the fusion trees.






% To find the best Steiner tree, we set the bottleneck $L^*$, in the original network graph, to a value and find the minimum-size Steiner tree over the modified graph. We repeat this process for all possible bottleneck values and pick the Steiner tree $\Steinerseet$ that yields the minimum latency. 





% More precisely, for a given edge $e\in E$, of the original graph $G=(V, E)$, we only include edges that have a latency equal or lower than the edge $e$ latency $T_e$. i.e. $G_e=(V, E_e=\{e' \in E \iff T_{e'} \leq T_e\})$. Now, we compute the Steiner tree for the modified graph $G_e$ for all the edges and pick the best one $\Steinerseet$.


==> 6--dp.tex <==
\section{\bf \red{Dynamic Programming Approaches (Whats the point?}}

\subsection{Dynamic Programming (\DP) Two-step Approach } 
Describe with equations and figures. Is there a performance guarantee?

\para{The first step} is to use \DP to \emph{independently} find the optimal swapping tree~\cite{swapping-tqe-22} for each adjacent pair of nodes in the given $\texttt{Path}(\udv)$.
Given a $\texttt{Path}(\udv)$ spanning $n$ number of nodes, we get $n-1$ number of swapping trees in the first step, each telling the minimum EP generation latency between a pair of adjacent nodes.
Since the swapping trees are constructed independently, the overall set of $n-1$ swapping trees may oversubscribe the resource at some nodes or links.
If the oversubscription happens, we split the resources equally\CZ{according to the rate ratio?} to meet the resource constraint.

\para{The second step} is another \DP that takes the output from the first step as the base case, then computes the minimal path graph state generation latency of $\texttt{Path}(\udv)$ from the bottom-up.

\softpara{Subproblem:}
Let $T[i,j]$ be the optimal expected latency of generating $\texttt{Path}(i \cdotp\cdotp j)$, $ u \leq i < j \leq v$ (\blue{the order of presence in the sequence of path graph state}), using a \red{fusion tree} over the path graph state nodes.

\softpara{Base case}: $T[i,j]$ for adjacent path graph state nodes $i,j$ is given by solutions from the first step.

\softpara{Equation:}
\begin{align}
    T[i,j] &= (\frac{3}{2}  B + t_c + t_{fr})/p_{fr} \\
    {\rm where:} & \nonumber \\
    B &= \min_{k \in V(\texttt{Path}(i\cdotp\cdotp j))}\max \big(T[i, k], T[k, j]) \nonumber
\end{align}

\softpara{Order of compute:} $|i-j|$ from $1$ to $(n-1)$

\softpara{Answer:} $T[u,v]$


\subsection{Improved \DP One-step Approach}

The higher-level idea is to do \DP only once.
To achieve it, we need to create a network path between $u$ and $v$, potentially including network nodes that are not in $V(\texttt{Path}(\udv))$.
In Fig.~\ref{fig:path-state} for example, such kind of network path for $V(\texttt{Path}(2\cdotp\cdotp 5))$ may be $[2,1,0,4,6,5]$ or $[2,3,0,4,6,5]$.

We first come up with a path-finding algorithm, which considers overlap. We use the Dijkstra algorithm to find the shortest path between all the two neighboring nodes in the path graph state, one for a time. Each time we find a shortest path, we delete the edges used to form a new graph, we then find the next shortest path in the new graph. Finally, we form the path by concatenating all the shortest paths. In this way, there will be no overlap in the path, however, we may not be able to find such a path, then we redo the pathfinding without deletion of edges and split the EP generation rate at the edges that are used more than once equally to the edges used it in the path.
\blue{Describe the pathfinding algorithm}
\vspace{0.5in}

We use $\texttt{Path}(x \cdotp\cdotp i \cdotp\cdotp j \cdotp\cdotp y)$ to denote a path graph state that is composed of $\texttt{Path}(i \cdotp\cdotp j)$ as the main part, while extending to node $x$ on $i$'s side and extending to node $y$ on $j$'s side, $x,y \notin V(\texttt{Path}(\udv))$ and $x,y \in V$.

If there is no extension, then $x,y$ is $null$,
if there is only one terminal node in $\texttt{Path}$, we let $i$ be the terminal node, 
if there is only one non-terminal extending node, we let $i$ be the terminal node.
And when there are less than two terminal nodes in $\texttt{Path}$, we assume that $x<y$ when $y \neq null$. For example, if there is only one terminal node and one non-terminal extending node in the $\texttt{Path}$, we use $T[x,i,null,null]$ to represent its optimal expected latency.

\softpara{Subproblem:}
Let $T[x,i,j,y]$ be the optimal expected latency of generating $\texttt{Path}(x \cdotp\cdotp i \cdotp\cdotp j \cdotp\cdotp y)$, $ u \leq i < j \leq v$ (\blue{the order of presence in the sequence of path graph state}), using a \red{fusion tree} over the path graph state nodes.

\softpara{Base case}: $T[null,i,j,null]$, the link EP generation latency for adjacent nodes $i,j$ in the quantum network.

\softpara{Equation}:
\begin{align}
    T[x,i,j,y] &= (\frac{3}{2}  B + t_c + t_{fd})/p_{fd} \\
    {\rm where:} & \nonumber \\
    B &= \min_{k \in V(\texttt{Path}(i\cdotp\cdotp j))}\max \big(T[x,i,k,z], T[z,k+1,j,y]) \nonumber
\end{align}

\softpara{Order of compute}:
$|i-j|$ from $1$ to $(n-1)$, and $x,y$ iterating over all nodes $\notin V(\texttt{Path}(\udv))$

\softpara{Answer}: $T[null,u,v,null]$

\softpara{Dealing with special cases}:

\blue{lots of equations...}
% \begin{enumerate}
%   \item 
%   $T[x, i, j, y]=\frac{3}{2}\max (T[x, i, k, z], T[z, k+1, j, y])$
%   \item 
%   $T[x, i, j, y]=\frac{3}{2}\max (T[x, i, k, null], T[null, k, j, y])$
%   \item 
%   $T[x, i, j, y]=\frac{3}{2}\max (T[x, null, null, z], T[z, i, j, y])$
%   \item 
%   $T[x, i, j, y]=\frac{3}{2}\max (T[x, i, j, z], T[z, null, null, y])$
%   \item 
%   $T[null, i, j, null]=\frac{3}{2}\max (T[z, i, null, null], T[z, j, null, null])$
%   \item 
%   $T[x, i, j, y]=\frac{3}{2}\max (T[x, i, k, null], T[null, k, j, y])$
%   \item 
%   $T[x, i, j, y]=\frac{3}{2}\max (T[x, i, j-1, z], T[z, j, null, y])$
%   \item 
%   $T[x, i, j, y]=\frac{3}{2}\max (T[x, i, null, z], T[z, i+1, j, y])$
%   \item 
%   $T[x, i, null, y]=\frac{3}{2}\max (T[x, i, null, z], T[z, null, null, y])$
%   \item 
%   $T[x, i, null, y]=\frac{3}{2}\max (T[x, null, null, z], T[z, i, null, y])$
%   \item 
%   $T[x, i, null, y]=\frac{3}{2}\max (T[x, i, null, null], T[y, i, null, null])$
%   \item
%   $T[x, null, null, y]=\frac{3}{2}\max (T[x, null, null, z], T[z, null, null, y])$
% \end{enumerate}

\vspace{0.5in}

==> 6a-fidelity.tex <==
% \section{\bf Incorporating Node and Fidelity Constraints} 
% \label{sec:fidelity}

% We now discuss changes to the algorithms to incorporate the node and fidelity constraints of the graph state fusion problem.


% \para{Node Constraints.} 
% \vspace{7cm}


% \para{Fidelity Constraints.} 
% \vspace{7cm}

% We now discuss changes to the algorithms to incorporate the node and fidelity constraints of the \ghzsr problem formulation in \S\ref{sec:formulation}. 

% \para{Node Constraints.}
% Recall that the node constraints are incorporated in the LP of the second step of the \fro algorithm. 
% %%%%
% In addition, the node-constraints are also somewhat incorporated in the first step of the \fro algorithm, 
% by assigning weights to terminal-pairs based on generation latency using an optimal swapping tree
% which incorporates node-constraints for each pair of nodes~\cite{swapping-tqe-22} .
% %%%%%%%%%%%%%%%%
% We incorporate node constraints in the \gf algorithm as follows.
% %%%%%%%%%%%%
% In the first step of the \gf algorithm, where we compute the best Steiner tree, we incorporate the node constraints as in the \fro's first step---i.e., by assignment weights to links based on generation 
% latency using an optimal swapping tree~\cite{swapping-tqe-22}.
% %%%%%%%%%%%%%
% In addition, in the second step of the \gf algorithm, wherein we compute a balanced fusion tree based on
% equi-{\it latency} division, we can further incorporate node constraints in determining the
% maximum generation latency of a link in a subtree.

% \para{Fidelity Constraints.} 
% We now discuss how to incorporate the fidelity constraints as defined in the \ghzsr problem formulation in \S\ref{sec:formulation}. Recall that the fidelity constraint is represented as a combination 
% of (i) memory storage time (age) threshold of \fidd, and (ii) number of leaves (operations-related fidelity)
% threshold of \fidl. We discuss these thresholds below.
% %%%%%%%%%%%%%%%%%%%%

% \softpara{Enforcing Age Threshold \fidd.}
% We start with discussing how we can incorporate the constraint of the expected age of any qubit to be 
% at most \fidd during generation of a \ghz state, while constructing the fusion tree. 
% %%%%%%%%%%

% In the {\bf FRO scheme}, the age of a qubit comes from two processes: (i) \eps generation for a terminal-pair using a swapping tree, and (ii) \ghz generation from \epss using a fusion tree. We divide the total
% age threshold \fidd into two thresholds, viz., $\fidd^s$ and $\fidd^f$, for swapping tree and fusion tree respectively, based on the relative heights of an average swapping tree and the fusion tree. 
% The swapping-tree age threshold  $\fidd^s$ can be enforced in determining the swapping trees as per~\cite{swapping-tqe-22}, while the fusion-tree age threshold $\fidd^f$ can be enforced 
% while constructing a fusion tree as follows. 
% %%%%%%%%%%%%%
% Recall that the \fro algorithm uses a DP algorithm to construct a fusion tree. Enforcing age threshold in the DP algorithm is relatively straightforward, by including an additional threshold-parameter 
% in the $L[\ ]$ function (see Eqn.~\ref{eqn:retain-dp}) and filtering out fusion trees 
% that violate the threshold parameter; determination of the threshold-parameter 
% of subtrees from that of a parent's node can be done as in~\cite{swapping-tqe-22}.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In the {\bf GF scheme,} a qubit ages purely due to \ghz generation using a fusion tree from link \epss. 
% Since we consider only balanced fusion trees in the second step of \gf, we can transform the age threshold approximately into a threshold on the height of the fusion tree---which is, in turn, a
% function of the size of the Steiner tree computed in the first step. 
% The size of the Steiner tree can be easily constrained in the Step 1's algorithm, 
% at the cost of a possibly higher generation latency of the bottleneck link.

% \softpara{Enforcing Operation Threshold \fidl.}
% For the {\bf FRO scheme}, the \fidl threshold can be enforced similar to the above age threshold, by 
% dividing the threshold into swapping and fusion trees, 
% handling swapping-tree threshold over number of 
% leaves as per~\cite{swapping-tqe-22}, and finally, 
% enforcing the number of leaves constraint in the 
% fusion tree by restricting its height in the DP approach.
% %%%%%%%%%%%%%
% For the {\bf GF scheme}, enforcing the \fidl threshold essentially amounts to
% restricting the number of leaves of the fusion tree, which 
% can be easily done by restricting the size of the Steiner tree 
% as we only consider balanced fusion trees. 

==> 7a-figures.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/with_one_side_path_vary_4_parameters_analytical.png}
    \caption{Generation Rates (from the linear program) for {\bf path} graph states for various schemes, for varying parameter values. (\oslp takes exorbitant computation time for a 100-node network. Thus, we plot \llp LP scheme; \rlp LP scheme has similar performance and not shown.)}
    \vspace*{-0.1in}
    \label{fig:path-lp}
\end{figure*}

\begin{figure*}
    \vspace{-0.05in}
    \centering
    \includegraphics[width=\textwidth]{figures/tree_vary_4_parameters.png}
    \vspace{-0.1in}
    \caption{Generation Rates (from the linear program) for {\bf tree} graph states for various schemes, for varying parameter values. In (c), for 15-21 terminals, \oslp has a generation rate of 0.04-0.03, \tslp have rates of 0.009-0.0007, while \ghzt and \central have rates of 0.005-0.0005 and $10^{{-}6}$-$10^{{-}8}$ respectively.}
    \label{fig:tree-lp}
    \vspace*{-0.25in}
\end{figure*}



==> def_new.tex <==
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{color}

\usepackage{subcaption}
\definecolor{accessbl}{cmyk}{1, 0.4, 0.3, 0}
\DeclareCaptionFont{bl}{\color{accessbl}}
\captionsetup[figure]{labelfont={bf,footnotesize, bl}, skip=0pt, labelsep=period, textfont={footnotesize}}

% *********************
% \usepackage{tcolorbox}
\usepackage{epsfig,endnotes,paralist,multirow}
\usepackage{wrapfig}
\usepackage{epsfig}
\usepackage[normalem]{ulem}
\usepackage{url}
\usepackage{soul}
\usepackage{multirow}
\usepackage{array}

% \usepackage{align}
% \usepackage{IEEEeqnarray}
% \usepackage{appendix}

\def\includeComments{include}
\def\includ{include}
\def\comm[#1]{\ifx\includeComments\includ  \bl \texttt{\textbf{\textit{Note: #1}}} \par \fi}
\def\inlinecomm[#1]{\ifx\includeComments\includ  \textit{Note: #1} \fi}

% *********************

% \usepackage{IEEEeqnarray}

\newcommand{\red}[1]{\textcolor{black}{#1}}
\newcommand{\blx}[1]{\textcolor{black}{#1}}
\newcommand{\bleu}[1]{\textcolor{black}{#1}}
\newcommand{\blue}[1]{\textcolor{black}{#1}}
\newcommand{\tqbl}[1]{\textcolor{black}{#1}}

\newcommand{\para}[1]{\smallskip \noindent {\bf #1}}
\newcommand{\softpara}[1]{\smallskip \noindent \underline{#1}}
% \newenvironment{prf}{{\em Proof:} \nopagebreak }{{\hfill$\blackbox$}}
\newcommand{\vsp}{\vspace{0.01in}}
\newcommand{\cw}{\color{white}}
\newcommand{\cb}{\color{black}}
\newcommand{\cbl}{\color{black}}
\newcommand{\cbr}{\color{red}}
\newcommand{\rb}[1]{\textcolor{black}{#1}}
\newcommand{\rbl}{\color{red}}

\def\blackbox{\hfill {\vrule height6pt width6pt depth0pt}}


\newcounter{theorem}
\newtheorem{thm}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{formula}{Formula}
\newtheorem{problem}{Problem}
\newtheorem{corollary}{Corollary}
\newtheorem{Plain}{}
\newtheorem{defin}{Definition}
\newtheorem{ex}{Example}
\newtheorem{lem}{Lemma}
\newtheorem{ob}{Observation}
%%\newtheorem{alg}{Algorithm}

\newenvironment{theorem}{\vsp \begin{thm} \nopagebreak}{{\hfill$\blackbox$} \end{thm} \vsp}
\newenvironment{thm-prf}{\vsp \begin{thm} \nopagebreak}{\end{thm}}
\newenvironment{lemma}{\vsp \begin{lem} \nopagebreak}{{\hfill$\blackbox$} \end{lem} \vsp}
\newenvironment{lem-wo-prf-box}{\vsp \begin{lem} \nopagebreak}{\end{lem}}
\newenvironment{lem-prf}{\vsp \begin{lem} \nopagebreak}{\end{lem}}
\newenvironment{prf}{{\em Proof:} \nopagebreak }{{\hfill$\blackbox$}}
\newenvironment{definition}[1]{\vsp\begin{defin}\begin{rm}(\textsc{#1})} {{\hfill$\Box$} \end{rm}\end{defin} \vsp}
\newenvironment{example}{\begin{ex} \nopagebreak \begin{rm}}{{\hfill$\Box$} \end{rm}\end{ex}}
\newenvironment{observation}{\noindent \begin{ob}}{{\hfill$\Box$}\end{ob}}
\newenvironment{cor-prf}{\vsp \begin{corollary} \nopagebreak}{\end{corollary}}
\newenvironment{cor}{\vsp \begin{corollary} \nopagebreak}{{\hfill$\Box$} \end{corollary} \vsp}
